Solving Hard Coreference Problems

Coreference resolution is a key problem in natural language understanding that still escapes reliable solutions. One fundamental difficulty has been that of resolving instances involving pronouns since they often require deep language understanding and use of background knowledge. In this paper, we propose an algorithmic solution that involves a new representation for the knowledge required to address hard coreference problems, along with a constrained optimization framework that uses this knowledge in coreference decision making. Our representation, Predicate Schemas, is instantiated with knowledge acquired in an unsupervised way, and is compiled automatically into constraints that impact the coreference decision. We present a general coreference resolution system that significantly improves state-of-the-art performance on hard, Winograd-style, pronoun resolution cases, while still performing at the state-of-the-art level on standard coreference resolution datasets.

==> 7.conclusion.tex <==
%In this paper, we propose and design Predicate Schemas to represent the knowledge needed for coreference.
%Automatically generate constraints for coreference during inference based on acquired knowledge and context.
%Put hard pronoun resolution problems into the scope of standard coreference and develop a system which can work for both tasks.
